Fitting Distances by Tree Metrics Minimizing the Total Error within a Constant Factor

We consider the numerical taxonomy problem of fitting a positive distance function ${D:{S\choose 2}\rightarrow \mathbb R_{>0}}$ by a tree metric. We want a tree $T$ with positive edge weights and including $S$ among the vertices so that their distances in $T$ match those in $D$. A nice application is in evolutionary biology where the tree $T$ aims to approximate the branching process leading to the observed distances in $D$ [Cavalli-Sforza and Edwards 1967]. We consider the total error, that is the sum of distance errors over all pairs of points. We present a deterministic polynomial time algorithm minimizing the total error within a constant factor. We can do this both for general trees, and for the special case of ultrametrics with a root having the same distance to all vertices in $S$. The problems are APX-hard, so a constant factor is the best we can hope for in polynomial time. The best previous approximation factor was $O((\log n)(\log \log n))$ by Ailon and Charikar [2005] who wrote "Determining whether an $O(1)$ approximation can be obtained is a fascinating question".

==> further_related_work.tex <==

\mtcom{From this point I mostly steal from the intro of Ailon-Charikar and adding their result.}
Further related work include the result of Ma et al. \cite{15ac-DBLP:journals/jco/MaWZ99} who considered the problem of finding the best
$L_p$ fit by an ultrametric where distances in the ultrametric
are no smaller that the given data. For this problem, they
obtained an $\calO(n^{1/p})$ approximation. Later, Dhamdhere \cite{6ac-DBLP:conf/approx/Dhamdhere04} considered the problem of finding a line metric to minimize additive distortion from the given data
(measured by the $L_1$ norm) and obtained an $\calO(\log n)$ approximation. In fact, his motivation for considering this
problem was to develop techniques that might be useful for finding the closest tree metric with distance measured by the
$L_1$ norm. Harp, Kannan and McGregor \cite{12ac-DBLP:conf/approx/HarbKM05} developed a factor
$\calO(\min\{n,k\log n\}^{1/p})$ approximation for the closest general tree metric under the $L_p$ norm where $k$ is the number
of distinct distances in the input.
\mtcom{I am pretty sure that they only get $k$-bound for ultrametrics. The reduction from tree metrics may introduce $k^2$ distances in the distance matrix for ultrametrics. I asked McGregor, and he thinks I might be right... Generally, since we have early that ultrametric implies tree metric, we could simplify the whole discussion by just talking about ultrametric...}



Of course, there is rich
literature on metric embedding problems where the measure of interest is the multiplicative distortion. Several
such problems have been studied in the context of approximating metric spaces via tree metrics (e.g. \cite{8ac-DBLP:journals/jcss/FakcharoenpholRT04}).
Researchers have also studied reconstruction of phylogenies under stochastic models of evolution (see Mossel
et al. \cite{16ac-DBLP:conf/stoc/MosselR05} and the references therein).
\vincent{
Cite: 
Rishi Sonthalia, Anna C. Gilbert:
Tree! I am no Tree! I am a low dimensional Hyperbolic Embedding. NeurIPS 2020;
Chenglin Fan, Anna C. Gilbert, Benjamin Raichel, Rishi Sonthalia, Gregory Van Buskirk:
Generalized Metric Repair on Graphs. SWAT 2020: 25:1-25:22
}
